Decoding the Silent Majority: Inducing Belief Augmented Social Graph with Large Language Model for Response Forecasting

Automatic response forecasting for news media plays a crucial role in enabling content producers to efficiently predict the impact of news releases and prevent unexpected negative outcomes such as social conflict and moral injury. To effectively forecast responses, it is essential to develop measures that leverage the social dynamics and contextual information surrounding individuals, especially in cases where explicit profiles or historical actions of the users are limited (referred to as lurkers). As shown in a previous study, 97% of all tweets are produced by only the most active 25% of users. However, existing approaches have limited exploration of how to best process and utilize these important features. To address this gap, we propose a novel framework, named SocialSense, that leverages a large language model to induce a belief-centered graph on top of an existent social network, along with graph-based propagation to capture social dynamics. We hypothesize that the induced graph that bridges the gap between distant users who share similar beliefs allows the model to effectively capture the response patterns. Our method surpasses existing state-of-the-art in experimental evaluations for both zero-shot and supervised settings, demonstrating its effectiveness in response forecasting. Moreover, the analysis reveals the framework's capability to effectively handle unseen user and lurker scenarios, further highlighting its robustness and practical applicability.

==> 2task.tex <==



==> 3data.tex <==


{\renewcommand{\arraystretch}{1} 
\begin{table}[t]
\begin{small}
	\centering
    \begin{tabular}{l|ccc}
   \toprule
Split & Train & Dev. & Test \\\midrule
\# Samples & 10,977  & 1,341 & 1,039 \\
\# Headlines & 3,561 & 1,065 & 843 \\
\# Users & 7,243 & 1,206  & 961 \\
Avg \# Profile Tokens &10.75  & 11.02 & 10.50 \\
Avg \# Response Tokens & 12.33 & 12.2 & 11.87 \\
Avg \# Headline Tokens &19.79  &  19.82& 19.72 \\\bottomrule 
\end{tabular}
    
    \caption{Summary statistics for the dataset.}
	\label{tab:data_stats}
	\vskip -0.3 in
\end{small}
\end{table}
}




    


\begin{table*}[]
\begin{small}
\centering
\begin{tabular}{lllllllllll}
\toprule
 & \multicolumn{6}{c}{\textbf{Textual Response}} & \multicolumn{2}{c}{\textbf{$\phi_{int}$}} & \multicolumn{2}{c}{\textbf{$\phi_{p}$}} \\
Name & \textcolor{violet}{BLEU}& \textcolor{violet}{BScore} &\textcolor{violet}{Meteor} & \textcolor{violet}{R-1} &\textcolor{violet}{R-L} & \multicolumn{1}{c|}{\textcolor{violet}{Avg. Len}} &\multicolumn{1}{c}{\textcolor{orange}{$r_s$}} & \multicolumn{1}{c|}{\textcolor{orange}{$r$}} & \teal{MiF1} & \teal{MaF1} \\ \midrule


Majority & - & - & - & - & - & \multicolumn{1}{c|}{-} & - & \multicolumn{1}{c|}{-} & 43.41 & 20.18 \\
Random & - & - & - & - & - & \multicolumn{1}{c|}{-} & 0.62 & \multicolumn{1}{c|}{0.41} & 35.51 & 30.55\\
GPT2 & 1.59 & -5.78 & 3.36 & 6.50 & 1.90 & \multicolumn{1}{c|}{9.64} & 50.34 & \multicolumn{1}{c|}{49.78} & 60.25 & 56.85 \\
T5 & 6.95 & -5.71 & 5.98 & \textbf{10.40} & \textbf{2.70} & \multicolumn{1}{c|}{18.87} & 50.06 & \multicolumn{1}{c|}{49.26} & 63.72 & 57.85 \\
BART & \textbf{8.17} & \textbf{-5.67} & \textbf{6.09} & 9.90 & 2.50 & \multicolumn{1}{c|}{\textbf{21.05}} & \textbf{62.03} & \multicolumn{1}{c|}{\textbf{61.82}} & \textbf{67.85} & \textbf{63.23} \\
BART w/o Profile & 7.30 & -5.70 & 5.91 & 10.00 & 2.50 & \multicolumn{1}{c|}{19.47} & 57.95 & \multicolumn{1}{c|}{58.20} & 67.28 & 62.26 \\
BART w/o History & 5.24 & -5.88 & 4.41 & 7.70 & 1.50 & \multicolumn{1}{c|}{18.62} & 48.80 & \multicolumn{1}{c|}{48.63} & 59.00 & 53.29 \\
BART w/o Both & 3.90 & -5.92 & 4.00 & 7.90 & 1.80 & \multicolumn{1}{c|}{15.73} & 45.28 & \multicolumn{1}{c|}{44.75} & 61.41 & 46.01 \\



 \bottomrule

\end{tabular}
\caption{Response forecasting results above show that the state-of-the-art models can predict responses with reasonable performance. The best overall performance is in bold.}
\label{tab:main}
\end{small}
\end{table*}









\section{Dataset Collection}
\label{sec:dataset}
		
In this section, we describe how we construct data from Twitter. Specifically, we used Twitter API\footnote{\url{developer.twitter.com/en/docs/twitter-api}} to crawl news headlines and comments below each headline from CNN Breaking News\fu{twitter.com/cnnbrk}, which is one of the most popular news accounts on Twitter. \heng{if you are using the same data set from ACL paper, then you can delete this paragraph}



\noindent\textbf{Preprocessing}. 
We collected news headlines and corresponding comments from CNN Breaking News between January 2017 and January 2019 and removed the comments that are over 50 tokens to avoid spamming. We stripped away HTML syntax tokens and normalized user reference with special tokens ``@user''.






\subsection{Persona Data}

We refer to the users who produce comments as responders. To describe responders, we collected different classes of persona attributes from Twitter. Specifically, we collected (1) User Profile, which is a short paragraph describing the user, and (2) User History, which are tweets written directly by the user. For user historical posts, to ensure that future posting activities are not included when predicting the comment, we collect the historical posts prior to the earliest data sample in our dataset for each individual user. 










 
\subsection{Annotation}
We obtained 14k headline and comment pairs from preprocessing. In the annotation stage, we collect labels for sentiment intensity and polarity of comments based on the context of the headline. For the 10k training instances, we produce automatic labels using deep-learning models trained on existing message-level datasets. More specifically, we train a Deberta-based model\ct{deberta} using data from SemEval-2018 Task 1\footnote{\url{https://competitions.codalab.org/competitions/17751}} \ct{mohammad2018semeval}, reaching over 85\% Pearson correlation. We then proceed to use crowd-sourcing to annotate the remaining 2k samples as our evaluation set. \heng{if this is repeating ACL paper's then remove it. otherwise you are disclosing author identity}

\noindent\textbf{Task Setup}. The annotation for the evaluation set is performed using the Amazon Mechanical Turk (MTurk) crowd-sourcing platform. The workers were each asked to annotate a headline and comment pair with three workers assigned to each data sample.  During the annotation, the annotator is asked to select the sentiment polarity label and the intensity of the sentiment based on their understanding of the input. The workers select positive, negative, or neutral for the sentiment polarity label and select on the integer scale of 0 to 3 for intensity. Four hundred and fifteen workers participated in this task in total and all annotators are paid a fair wage above the federal minimum.


\noindent\textbf{Quality Control}. To ensure the quality of annotation, we allowed only the workers who have at least 95\% approval rate and have had at least 5,000 hits approved to access our tasks. We further removed workers who have a <70\% accuracy in the first 30 annotations and discarded the assignments that have completion time deviated from the expected average largely. We used majority voting to determine the final labels: if at least two annotators agreed on a label, we chose it as the final label. The resulting annotated samples achieve an inter-annotator agreement accuracy of 81.3\%. We show the statistics of the dataset in Table~\ref{tab:data_stats}.




























